High contrast dual-mode optical and 13C magnetic resonance imaging in diamond particles

Multichannel imaging -- the ability to acquire images of an object through more than one imaging mode simultaneously -- has opened interesting new perspectives in areas ranging from astronomy to medicine. Visible optics and magnetic resonance imaging (MRI) offer complementary advantages of resolution, speed and depth of penetration, and as such would be attractive in combination. In this paper, we take first steps towards marrying together optical and MR imaging in a class of biocompatible particulate materials constructed out of diamond. The particles are endowed with a high density of quantum defects (Nitrogen Vacancy centers) that under optical excitation fluoresce brightly in the visible, but also concurrently electron spin polarize. This allows the hyperpolarization of lattice 13C nuclei to make the particles over three-orders of magnitude brighter than in conventional MRI. Dual-mode optical and MR imaging permits immediate access to improvements in resolution and signal-to-noise especially in scattering environments. We highlight additional benefits in background-free imaging, demonstrating lock-in suppression by factors of 2 and 5 in optical and MR domains respectively. Ultimate limits could approach as much as two orders of magnitude in each domain. Finally, leveraging the ability of optical and MR imaging to simultaneously probe Fourier-reciprocal domains (real and k-space), we elucidate the ability to employ hybrid sub-sampling in both conjugate spaces to vastly accelerate dual-image acquisition, by as much as two orders of magnitude in practically relevant sparse-imaging scenarios. This is accompanied by a reduction in optical power by the same factor. Our work suggests interesting possibilities for the simultaneous optical and low-field MR imaging of targeted diamond nanoparticles.

==> supplement_fig/Commands3.tex <==
\newcommand{\inset}{\hspace{10pt}}
\newcommand{\vs}{\vspace{10pt}}
% Math symbols
\newcommand{\itwo}{{\frac1{2}}}
\newcommand{\ist}{{\frac1{\sqrt{2}}}}
\newcommand{\id}{\mathds{1}}
\newcommand{\half}{\frac{1}{2}}
% Greek small
\newcommand{\xa}{\alpha}
\newcommand{\cc}{{\cal C}}
\newcommand{\hb}{\hbar}
\newcommand{\xb}{\beta}
\newcommand{\xc}{\chi}
\newcommand{\xd}{\delta}
\newcommand{\xe}{\epsilon}
\newcommand{\angstrom}{\mbox{\normalfont\AA}}

%\newcommand{\xe}{\upvarepsilon}
\newcommand{\xg}{\gamma}
\newcommand{\xt}{\theta}
\newcommand{\ot}{\otimes}
\newcommand{\xn}{\eta}
\newcommand{\xk}{\kappa}
\newcommand{\xl}{\lambda}
\newcommand{\xr}{\rho}
\newcommand{\xo}{\omega}
\newcommand{\xph}{\phi}
\newcommand{\xps}{\psi}
\newcommand{\nb}{\nabla}
\newcommand{\xvph}{\varphi}
\newcommand{\xs}{\sigma}
\newcommand{\xz}{\zeta}
\newcommand{\pp}{\perp}
\newcommand{\app}{\approx}
\newcommand{\dw}{\downarrow}
\newcommand{\up}{\uparrow}
\newcommand{\Cs}{{}^{13}\R{C}}
\newcommand{\Ns}{{}^{14}\R{N}}
\newcommand{\Hs}{{}^{1}\R{H}}

\newcommand{\mG}[0]{\mathcal{G}}
\newcommand{\mR}[0]{\mathcal{R}}
\newcommand{\bB}[0]{\mathbf B}
\newcommand{\bs}[0]{\mathbf \sigma}
\newcommand{\bH}[0]{\mathbf H}
\newcommand{\bn}[0]{\hat{\mathbf n}}

\newcommand{\ltrt}{\leftrightarrow}
\newcommand{\iso}[1]{{}^{#1}}
\newcommand{\V}[1]{\vec{#1}}
%\newcommand{\mc}[1]{\mathcal{#1}}

\newcommand{\sinc}{\R{sinc}}
\newcommand{\rect}{\R{rect}}

\newcommand{\spl}[1]{\begin{align}\begin{split} #1 \end{split} \end{align}}

% Greek large
\newcommand{\xA}{\Alpha}
\newcommand{\xB}{\Beta}
\newcommand{\xD}{\Delta}
\newcommand{\xE}{\Epsilon}
\newcommand{\xG}{\Gamma}
\newcommand{\xT}{\Theta}
\newcommand{\xN}{\Eta}
\newcommand{\xK}{\Kappa}
\newcommand{\xL}{\Lambda}
\newcommand{\xO}{\Omega}
\newcommand{\xPh}{\Phi}
\newcommand{\xPs}{\Psi}
\newcommand{\xS}{\Sigma}
\newcommand{\Spl}[1]{\begin{align*}\begin{split} #1 \end{split} \end{align*}}


\newcommand{\mP}[0]{\mathcal{P}}
\newcommand{\mU}[0]{\mathcal{U}}
\newcommand{\bp}[0]{\mathbf p}
\newcommand{\bq}[0]{\mathbf q}
\newcommand{\bP}[0]{\mathbf P}
\newcommand{\bb}[0]{\mathbf b}

\newcommand{\bA}[0]{\mathbf A}
\newcommand{\bS}[0]{\mathbf S}
\newcommand{\bI}[0]{\mathbf I}
%\newcommand{\bB}[0]{\mathbf B}
\newcommand{\bxO}[0]{\mathbf \Omega}
\newcommand{\bM}[0]{\mathbf M}
\newcommand{\be}[0]{\mathbf e}
\newcommand{\bu}[0]{\mathbf u}
\newcommand{\bv}[0]{\mathbf v}
\newcommand{\bR}[0]{\mathbf R}
\newcommand{\bx}[0]{\hat{\mathbf x}}
\newcommand{\by}[0]{\hat{\mathbf y}}
\newcommand{\bz}[0]{\hat{\mathbf z}}
\newcommand{\br}[0]{\hat{\mathbf r}}
\newcommand{\balpha}[0]{\boldsymbol \alpha}
\newcommand{\bdelta}[0]{\boldsymbol \delta}
\newcommand{\al}[1]{\begin{align} #1 \end{align}}

% other useful commands
\newcommand{\fr}[2]{\frac{#1}{#2}}
\newcommand{\ov}[1]{\overline{#1}}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\dwt}[1]{\widetilde{\widetilde{#1}}}
\newcommand{\h}[1]{\hat{#1}}
\newcommand{\s}[2]{\sum_{#1}^{#2}}
\newcommand{\zi}[2]{\int_{#1}^{#2}}
\newcommand{\sq}[1]{\sqrt{#1}}
\newcommand{\zd}{\cdot}

\newcommand{\mH}[0]{\mathcal{H}}
\newcommand{\mF}[0]{\mathcal{F}}
\newcommand{\mT}[0]{\mathcal{T}}
\newcommand{\mB}[0]{\mathcal{B}}

\newcommand{\rt}{\rightarrow}
\newcommand{\lt}{\leftarrow}
\newcommand{\xrt}[1]{\xrightarrow{#1}}
\newcommand{\Rt}{\Rightarrow}
\newcommand{\xinf}{\infty}
\newcommand{\op}{\oplus}
\newcommand{\oti}{\otimes}
\newcommand{\e}{\exp}
\newcommand{\dg}{\dagger}

\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
                  
\newcommand{\benum}{\begin{enumerate}}
\newcommand{\eenum}{\end{enumerate}}
                    
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}}


\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}

\newcommand{\bev}{\begin{verbatim}}
\newcommand{\eev}{\end{verbatim}}

\newcommand{\code}[1]{\texttt{#1}}

\newcommand{\non}{\nonumber}
\newcommand{\noi}{\noindent}
\newcommand{\cd}{\cdots}
\newcommand{\zt}{\times}

\newcommand{\qt}{\tau}

% brackets
\newcommand{\lb}{\left(}
\newcommand{\rb}{\right)}
\newcommand{\lsb}{\left[}
\newcommand{\rsb}{\right]}
\newcommand{\lcb}{\left\{}
\newcommand{\rcb}{\right\}}
\newcommand{\labs}{\left|}
\newcommand{\rabs}{\right|}
\newcommand{\lan}{\langle}
\newcommand{\ran}{\rangle}
\newcommand{\pll}{\parallel}
\newcommand{\ppp}{\perp}
\newcommand{\Rb}{${}^{87}$Rb\ }

%bold
\newcommand{\B}[1]{\mathbf{#1}}
\newcommand{\T}[1]{\textbf{#1}}
\newcommand{\I}[1]{\textit{#1}}
\newcommand{\R}[1]{\textrm{#1}}
%\newcommand{\Ir}[1]{\textit{\Rd{#1}}}
\newcommand{\IIr}[1]{\textit{\Rd{#1}}}

%\newcommand{\C}{\cdot}
\newcommand{\vv}{\vec}
\newcommand{\dov}[1]{\overline{\overline{#1}}}

%label and ref
\newcommand{\zl}[1]{\label{eqn:#1}}
\newcommand{\zr}[1]{Eq. (\ref{eqn:#1})}
\newcommand{\zfl}[1]{\protect\label{fig:#1}}
\newcommand{\zfr}[1]{Fig. \ref{fig:#1}}
\newcommand{\ztl}[1]{\label{table:#1}}
\newcommand{\ztr}[1]{Table \ref{table:#1}}
\newcommand{\zsl}[1]{\label{sec:#1}}
\newcommand{\zsr}[1]{Sec. \ref{sec:#1}}
\newcommand{\zal}[1]{\label{app:#1}}
\newcommand{\zar}[1]{Appendix \ref{app:#1}}




% For NV
\newcommand{\carb}{$^{13}$C }
% Quantum Kets
\newcommand{\ket}[1]{\left\vert{#1}\right\rangle}
\newcommand{\bra}[1]{\left\langle{#1}\right\vert}
\newcommand{\braket}[2]{\langle{#1}\vert{#2}\rangle}
\newcommand{\ketbra}[2]{\ket{#1}\bra{#2}}
\newcommand{\sand}[3]{\langle{#1}\vert#2\vert{#3}\rangle}
\newcommand{\expec}[1]{\left\langle #1\right\rangle}
\newcommand{\kpsi}{\vert{\psi}\rangle}
\newcommand{\kphi}{\vert{\phi}\rangle}
\newcommand{\kphit}{\vert{\phit}\rangle}
\newcommand{\bpsi}{\langle{\psi}\vert}
\newcommand{\bphi}{\langle{\phi}\vert}
\newcommand{\bphit}{\langle{\phit}\vert}
\newcommand{\ku}{\vert{0}\rangle}
\newcommand{\kd}{\vert{1}\rangle}
\newcommand{\kup}{\vert{\uparrow}\rangle}
\newcommand{\kdw}{\vert{\downarrow}\rangle}
%\newcommand{\bu}{\langle{0}\vert}
%\newcommand{\bd}{\langle{1}\vert}
\newcommand{\kk}{\vert{k}\rangle}
\newcommand{\bk}{\langle{k}\vert}
\newcommand{\ci}{\circ}
% Quantum Ops
\newcommand{\ave}[1]{\left\langle #1\right\rangle}
\newcommand{\vop}[1]{\hat{\vec{#1}}}
\newcommand{\comm}[2]{\left[{#1},{#2}\right]}
\newcommand{\ham}{{\mathcal{H}}}
%Pauli
\newcommand{\sone}{\mathds{1}}
\newcommand{\sx}{\sigma_x}
\newcommand{\sy}{\sigma_y}
\newcommand{\sz}{\sigma_z}
%\newcommand{\spl}{\sigma_+}
\newcommand{\sm}{\sigma_-}
% 2x2 Matrix
\newcommand{\mat}[4]{\left(\begin{array}{cc}{#1}&{#2}\\
{#3}&{#4}\end{array}\right)}
\newcommand{\matnob}[4]{\begin{array}{cc}{#1}&{#2}\\
{#3}&{#4}\end{array}}

\newcommand{\matthree}[9]{\left(\begin{array}{ccc}{#1}&{#2}&{#3}\\
{#4}&{#5}&{#6}\\
{#7}&{#8}&{#9}\end{array}\right)}

\newcommand{\ba}{\left\{ \begin{array}{lr}}
\newcommand{\ea}{\end{array}\right.}    

\newcommand{\coltwo}[2]{\left[\begin{array}{c}{#1}\\{#2}\end{array}\right]}


\newcommand{\diagfour}[4]{\left[\begin{array}{cccc}{#1}&{}&{}&{}\\
{}&{#2}&{}&{}\\
{}&{}&{#3}&{}\\
{}&{}&{}&{#4}
\end{array}\right]}

\newcommand{\diagthree}[3]{\left[\begin{array}{ccc}{#1}&{}&{}\\
{}&{#2}&{}\\
{}&{}&{#3}
\end{array}\right]}

\newcommand{\sect}[1]{\vspace{0.2in}
\noi\textbf{#1:\\}}             
 
%\newcommand{\bookjun}[1]{\href[page=#1]{../../notes/research/book-jun-2015.pdf}{Jun, page #1}}.
%\newcommand{\bookmay}[1]{\href[page={#1}]{../../notes/research/book-may-2015.pdf}{May, page {#1}}}.

\newcommand{\Bl}[1]{\textcolor{RoyalBlue}{#1}} %RoyalBlue MidnightBlue
\newcommand{\Rd}[1]{\textcolor{BrickRed}{#1}} %RoyalBlue MidnightBlue
%\newcommand{\Rd}[1]{\textcolor{Red}{#1}} %RoyalBlue MidnightBlue

% Trace
\newcommand{\Tr}[1]{\textrm{Tr}\left\{{#1}\right\}}
\newcommand{\tr}[1]{\textrm{Tr}\left\{{#1}\right\}}
\newcommand{\ptr}[2]{\textrm{Tr}_{#1}\left\{{#2}\right\}}
\newcommand{\pTr}[2]{\textrm{Tr}_{#1}\left\{{#2}\right\}}
\newcommand{\im}[1]{\textrm{Im}\left[{#1}\right]}
\newcommand{\re}[1]{\textrm{Re}\left[{#1}\right]}
\newcommand{\diag}{{\rm diag}}
% Derivative
\newcommand{\pdev}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\dev}[2]{\frac{d\, #1}{d\, #2}}
\newcommand{\del}{\partial}




% List
\newcommand{\blist}[1]{
 \begin{list}{#1}%$\ast\circ\bullet\Right
 \begin{align}
	 arrow
 \end{align}
 $\checkmark\star
  { \setlength{\itemsep}{3pt}
     \setlength{\parsep}{2pt}
     \setlength{\topsep}{3pt}
     \setlength{\partopsep}{0pt}
     \setlength{\leftmargin}{1em}
     \setlength{\labelwidth}{1em}
     \setlength{\labelsep}{0.5em} } }
\newcommand{\elist}{
  \end{list}  }     


\DeclareMathSymbol{\vartheta}{\mathalpha}{letters}{"12}
\DeclareMathSymbol{\theta}{\mathalpha}{letters}{"23}
\DeclareMathSymbol{\phi}{\mathalpha}{letters}{"27}
\DeclareMathSymbol{\varphi}{\mathalpha}{letters}{"1E}

\newcommand{\boxe}[2]
  {
\begin{center}
\noindent\framebox[#2in][c]{\begin{minipage}[c]{\columnwidth}#1\end{minipage}}% 
\end{center}
   }

\newcommand{\boxcolwidth}[1]
  {

   \noindent\fbox{\begin{minipage}[c]{\columnwidth}#1\end{minipage}}  }

\newcommand{\specialcell}[2][c]{%
  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}
	
	
\newcommand{\insfigsc}[3]
	{
	\begin{figure}[htbp]
\centering
\includegraphics[width=#3\linewidth]{#1}
\caption{#2}
\zfl{#1}
\end{figure}}

%\newcommand{\insfigscfull}[3]
%	{
%	\begin{figure*}[htbp!]
%\centering
%\includegraphics[width=#3\linewidth]{#1}
%\caption{#2 \zfl{#1}}
%\end{figure*}}


\newcommand{\insfigscfull}[3]
	{
	\begin{figure*}[htbp]
\centering
\includegraphics[width=#3\linewidth]{#1}
\refstepcounter{figure}
\smallskip\noindent\footnotesize  \begin{flushleft} Figure \thefigure: #2\zfl{#1}\end{flushleft}
\end{figure*}}

\newcommand{\bef}
{
\begin{figure}[htbp]
\centering
}

\newcommand{\eef}{\end{figure}}

\newcommand{\subfig}[2]
{
\subfigure[]{\includegraphics[width=#2\linewidth]{#1}\zfl{#1}}
}

%\newcommand{\subfig}[2]
%{
%\subfloat[]{
%\begin{minipage}[c][1\width]{ 0.5\textwidth} 
%\centering	
 %\includegraphics[width=#2\textwidth]{#1} 
%\end{minipage}} 
%\zfl{#1}}


\newcommand{\marfig}[2]
{
\begin{marginfigure}%
\centering
  \includegraphics[width=\linewidth]{#1}
  \caption{#2}
\zfl{#1}
\end{marginfigure}
}

\newcommand{\marfigsc}[3]
{
\begin{marginfigure}%
\centering
  \includegraphics[width=#3\linewidth]{#1}
  \caption{#2}
\zfl{#1}
\end{marginfigure}
}

\newcommand{\beg}{\begingroup
    \fontsize{8pt}{10pt}\selectfont}
\newcommand{\eeg}{\endgroup}
